Generating Band-Limited Adversarial Surfaces Using Neural Networks

Generating adversarial examples is the art of creating a noise that is added to an input signal of a classifying neural network, and thus changing the network's classification, while keeping the noise as tenuous as possible. While the subject is well-researched in the 2D regime, it is lagging behind in the 3D regime, i.e. attacking a classifying network that works on 3D point-clouds or meshes and, for example, classifies the pose of people's 3D scans. As of now, the vast majority of papers that describe adversarial attacks in this regime work by methods of optimization. In this technical report we suggest a neural network that generates the attacks. This network utilizes PointNet's architecture with some alterations. While the previous articles on which we based our work on have to optimize each shape separately, i.e. tailor an attack from scratch for each individual input without any learning, we attempt to create a unified model that can deduce the needed adversarial example with a single forward run.

==> chapters/acknowledgements.tex <==
\begin{acknowledgements}
Firstly, I want to thank somebody, and somebody else.\footnote{Here is a footnote} Here is another note.
\end{acknowledgements}

==> chapters/appendices.tex <==
% Writing appendices is super super easy in LaTeX. You just write
% \appendix to demarcate where the normal content ends and the appendices start. After \appendix, chapters (started with \chapter) are considered as appendices.
%
% In this example though, we're using the appendices environment. Long story short, this is because we want some fancy titles in the toc.
\begin{appendices}

% Appendix A
% ----------

\chapter{Some random python code}
This template includes the \texttt{minted} package, which allows you to import code and syntax highlight it. For example, the text below is imported directly from the \texttt{code/test.py} file using the \textbackslash\texttt{inputminted} command:

\begin{framed}
\inputminted{python}{code/test.py}
\end{framed}

And here is a snippet of Python with the \texttt{minted} environment:

\begin{framed}
\begin{minted}[breaklines]{python}
# Why don't you try running this?
# See what it does? hm?

m = [ 2, 3, 0, 1, 4 ];
x = [ 'rmdq', 'd', 'n`slk', 'odftp`v)', 'hdk' ];

c = ''.join(list(map(lambda y: chr(ord(y) ^ 5).upper() + ' ' if y != ' ' else '  ', ' '.join([ x[m[i]] for i, v in enumerate(x) ]))));

print('%s\r\n%s\r\n%s\r\n' % ('=' * len(c), c, '=' * len(c)));
\end{minted}
\end{framed}

\cleardoublepage
Minted supports many, many languages -- so you're not just limited to Python. For example, here's some random C++ code.

\begin{framed}
\begin{minted}[breaklines]{cpp}
void CTimesTable::Print(const int number, const int upTo) const
{
    for(int i = 1; i <= upTo; i++)
        printf("%d x %d = %d\r\n", number, i, number * i);
}
\end{minted}
\end{framed}







% Appendix B
% ----------

\chapter{Some other stuff}
Here is just an example of some other stuff.

% End of appendices
\end{appendices}

==> chapters/blank-pages.tex <==
% The blank page environment allows you to insert
% pages into your thesis for specific things

\begin{blankpage}
    \chapterTitle{A blank page}
    This is an optional page environment you could use for things like:
	\begin{itemize}
		\item Your own custom preamble chapters (use \texttt{\textbackslash chapterTitle} for titles!)
		\item \emph{``This work is dedicated to...''}
		\item A copyright notice
		\item Additional notes
		\item Quotes
		\item List of publications
		\item An actual blank page
		\item Nomenclature / glossaries, etc.
	\end{itemize}
	It is not recommended to use this in your undergraduate thesis for submission. It has been left in here to make you aware of its existence. This is largely because it does not follow the guidelines set out for undergraduate theses, but you could include this environment for your own personal printed copy. Consult with your supervisor to see if you can use it. 
	
	In addition, you can pass an optional parameter to this environment with the value \texttt{c} to centre this text vertically on the page (use the \texttt{center} environment to align horizontally).
\end{blankpage}

==> preamble/bib-setup.tex <==
% Add in the .bib files you wish to add 
% into your document here. If you want to
% include others, just copy this line and
% change the path!

%\addbibresource{bib/references.bib}
